Active Local Learning

In this work we consider active local learning: given a query point $x$, and active access to an unlabeled training set $S$, output the prediction $h(x)$ of a near-optimal $h \in H$ using significantly fewer labels than would be needed to actually learn $h$ fully. In particular, the number of label queries should be independent of the complexity of $H$, and the function $h$ should be well-defined, independent of $x$. This immediately also implies an algorithm for distance estimation: estimating the value $opt(H)$ from many fewer labels than needed to actually learn a near-optimal $h \in H$, by running local learning on a few random query points and computing the average error. For the hypothesis class consisting of functions supported on the interval $[0,1]$ with Lipschitz constant bounded by $L$, we present an algorithm that makes $O(({1 / \epsilon^6}) \log(1/\epsilon))$ label queries from an unlabeled pool of $O(({L / \epsilon^4})\log(1/\epsilon))$ samples. It estimates the distance to the best hypothesis in the class to an additive error of $\epsilon$ for an arbitrary underlying distribution. We further generalize our algorithm to more than one dimensions. We emphasize that the number of labels used is independent of the complexity of the hypothesis class which depends on $L$. Furthermore, we give an algorithm to locally estimate the values of a near-optimal function at a few query points of interest with number of labels independent of $L$. We also consider the related problem of approximating the minimum error that can be achieved by the Nadaraya-Watson estimator under a linear diagonal transformation with eigenvalues coming from a small range. For a $d$-dimensional pointset of size $N$, our algorithm achieves an additive approximation of $\epsilon$, makes $\tilde{O}({d}/{\epsilon^2})$ queries and runs in $\tilde{O}({d^2}/{\epsilon^{d+4}}+{dN}/{\epsilon^2})$ time.

==> Preliminaries.tex <==
% !TEX root = main.tex
\section{Notation}
%
\label{section:preliminaries}
For a positive integer n, let $[n]$ denote $\{1,2,\cdots,n\}$. For two positive semidefinite matrices $A$ and $B$, let $A\preceq B (\text{or } A\succeq B)$ denote that $B-A (\text{or } A-B)$ is a positive semidefinite matrix. We use $\tilde{O}$ notation to hide polylogarithmic factors in the input parameters and error rates. 
%
%
%
%

==> ShortRelatedWork.tex <==
% !TEX root = main.tex
\section{Related Work}
\label{section:related-work}
\textbf{Local Computation Algorithms: }Our work on locally learning Lipschitz functions closely resembles the concept of local computation algorithms introduced in the pioneering work of \cite{rubinfeld2011fast}. They were interested in the question of whether it is possible to compute specific parts of the output in time sublinear in the input size. As mentioned by the authors, that work was a formalization of different forms of this concept already existing in literature in the form of  local distributed computation, local algorithms,
locally decodable codes and local reconstruction models. The reader can refer to \cite{rubinfeld2011fast} for the detailed discussion of work in each of these subfields. In the paper, the authors looked at several graph problems in the local computation model like maximal independent set, $k$-SAT and hypergraph coloring. Since then, there has been a lot of further work on local computation algorithms for various graph problems including maximum matching, load balancing, set cover and many others (\cite{mansour2013local, alon2012space, mansour2012converting, parnas2007approximating,parter2019local,levi2014local, grunau2020improved}). There also has been work on solving linear systems locally in sublinear time \citep{andoni2018solving} for the special case of sparse symmetric diagonally dominant matrices with small condition number.  However, the primary focus of all of these works has been on sublinear computational complexity, whereas we focus primarily on sample complexity. Note that in principle if we can solve the linear program corresponding to the best Lipschitz function locally in sublinear time, we would also get sublinear sample complexity. However, the linear program for computing the best Lipschitz function has constraints and does not fit into their framework of solving linear systems.

\cite{mansour2014robust, feige2015learning} considered the use of local computation algorithms for inference settings.
However, the focus was on time complexity rather than sample complexity. The problem of computing a part of output of the learned function in sublinear sample complexity as compared to the usual notion of complexity of the function class (VC-dimension, covering numbers) has not been previously looked at in the literature to the best of our knowledge. For a detailed comparison to our results, the reader can refer to Appendix~\ref{appendix:relatedwork}. 
%
%

\textbf{Transductive Inference: }Another related line of work that has been done in the learning theory community is based on transductive inference \citep{vapnik1998statistical} which as opposed to inductive inference aims to estimate the values of the function on a few given data points of interest. The philosophy behind this line of work is to avoid solving a more general problem as an intermediate step to solve a problem. This idea is very similar to the idea considered here wherein we are interested in computing the prediction at specific query points of interest. However, our prediction algorithm still requires a guarantee on the total error over the complete domain with respect to the underlying distribution though it is never explicitly constructed for the entire domain unless required. The reader can refer to chapters 24 and 25 in \cite{chapelle2009semi} for additional discussion on the topic. 

\textbf{Property Testing: }There also has been a large body of work in the theoretical computer science community on property testing where the goal is to determine whether a function belongs to a class of functions or is far away from it with respect to some notion of distance in sublinear sample complexity. The commonly studied testing problems include testing monotonicity of a function over a boolean hypercube \citep{goldreich1998testing, chakrabarty2016n, chen2014new, khot2018monotonicity}, testing linearity over finite fields \citep{bellare1996linearity, ben2003randomness}, testing for concise DNF formulas \citep{diakonikolas2007testing, parnas2002testing} and testing for small decision trees \citep{diakonikolas2007testing}. However, all the aforementioned algorithms work in a query model where a query can be made on any arbitrary domain point of choice. 

The setting which is closer to learning  where the labels can only be obtained from a fixed distribution was first studied by \cite{goldreich1998property, kearns2000testing}.\includecomment{ kearns and rons 200 gave better sample complexity bounds for testing various problems like decisions trees and restricted form of neural networks than would be required for learning the best function in that class.} This setting is also called as passive property testing. The notion of active property testing was first introduced by \cite{balcan2012active} where an algorithm can make active label queries on an unlabeled sample of points drawn from an unknown distribution. However, one limitation of these algorithms is that they do not give meaningful bounds to distinguish the function from being approximately close to the function class (rather than belonging to the class) vs. far away from it. 

\cite{parnas2006tolerant} first introduced the notion of tolerant testing where the aim is to detect whether the function is $\epsilon$ close to the class or $2\epsilon$ far from it in the query model with queries on arbitrary domains points of choice. This also relates to estimating the distance of the function from the class within an additive error of $\epsilon$. \cite{blum2018active} first studied the problem of active tolerant testing where they were interested in algorithms which are tolerant to the function not being exactly in the function class and also have active query access to the labels over the unlabeled samples from an unknown distribution. Specifically, \cite{blum2018active}
gave algorithms for estimating the distance of the function from the class of union of $d$ intervals with a labeled sample complexity of $\text{poly}({1}/{\epsilon})$. The key point to be noted is that the labeled sample complexity is independent of $d$ which is the VC dimension of that class and dictates the number of samples required for learning. We note that our algorithm for error estimation for the class of Lipschitz functions in labeled sample complexity independent of $L$ is another work along these lines. 

Property testing has also been studied for the specific class of Lipschitz functions \citep{jha2013testing, chakrabarty2013optimal, berman2014lp}. However, all of these results either query arbitrary domain points or are in the non-tolerant setting or work only for discrete domain. 
%
%Another related notion called local reconstruction has been studied in \cite{jha2013testing, saks2010local} but none of them are directly applicable to our settings. The reader can refer to Appendix~\ref{} for a detailed comparison to our results,. 

A closely related work to our method of error estimation where the predicted label depends on the labels of the training data weighted according to some appropriate kernel function was also considered in \cite{blum2018active}. In particular, \cite{blum2018active} looked at the setting where the predicted label was based on the $k$-nearest neighbors and showed that the $\ell_{1}$ loss can be estimated up to an additive error of $\epsilon$ using $O({1}/{\epsilon^2})$ label queries on $N+O({1}/{\epsilon^2})$ unlabeled samples. Their results also extend to the case where the prediction is the weighted average of all the unlabeled points in the sample by sampling with a probability proportional to the weight of the point. However, this sampling when repeated for $O({1}/{\epsilon^d})$ number of different linear transformations would lead to a labeled sample complexity depending on ${1}/{\epsilon^d}$. Moreover, sampling a point with a probability proportional to the weight would require a running time of $N$ per query and thus, would give a total running time of $O({N}/{\epsilon^{d+2}})$. %However, we circumvent this issue and obtain a running time depending only on $\tilde{O}(\frac{N}{\epsilon^2}+\frac{\log(N)}{\epsilon^{d+2}})$ by using recent advances achieving faster algorithms for kernel density estimation \citep{backurs2018efficient}. 

==> extra.tex <==
We wish to estimate the value of the expected loss i.e. $E_{x,y \sim D}|\frac{\sum_i^NK(x_i,x)y_i}{\sum_i^NK(x_i,x)} - y|$. Our theorem stated below shows that it is possible to estimate this error in $O(\frac{1}{\epsilon^2})$ labelled queries and $\tilde{O}(d\text{poly}(\frac{\log(N)}{\epsilon}))$ running time. Note that if we compute the loss exactly for each of the sampled points $x$ from the distribution $D$, then we would need a total of $O(\frac{N}{\epsilon^2})$ labelled queries. If we instead decide to estimate the loss for each datapoint $x$ by subsampling points from the training data, if we sample proportional to $\frac{K(x_i,x)}{\sum_iK(x_i,x)}$, then we would need a total running time of $O(\frac{N}{\epsilon^2})$ since for each query point $x$, we would need to compute $\sum_iK(x_i,x)$. On the other hand, if we decide to sample the training points uniformly, then we would need 

\begin{theorem}
\label{thm:kdeerror}
Given the setting above, it is possible to estimate the error of the prediction function above i.e. $E_{x,y \sim D}|\frac{\sum_i^NK(x_i,x)y_i}{\sum_i^NK(x_i,x)} - y|$ upto accuracy $\epsilon$ with $O(\frac{1}{\epsilon^2})$ label queries and $O(\frac{d\log(N)^4}{\epsilon^4})\log(\frac{1}{\epsilon^2p})$ runtime with failure probability atmost $p$. 
\end{theorem}
\begin{proof}
Let $\frac{K(x_i,x)}{\sum_iK(x_i,x)} = p(x,x_i)$. It is easy to see that $\sum_ip(x,x_i) = 1 \quad \forall x \in R^d$. Then we can write the loss which we want to estimate as $E_{x,y \sim D}|\sum_i^Np(x_i,x)y_i - \sum_i^Np(x_i,x)y| = E_{x,y \sim D}\sum_i^Np(x_i,x)|y_i-y|$. From Lemma \ref{lemma:sampling_runtime}, we can sample a $x_i$ with probability proportional to $p(x_i,x)(1\pm\delta)$ for any fixed $x$ in running time $O(\frac{d\log(N)^4}{\delta^2})\log(\frac{1}{\epsilon^2p})$ with a failure probability of atmost $p\epsilon^2$. So now our estimator for this error is the following: we take $ M = O(\frac{1}{\epsilon^2})$ independent  random samples $\{x_i\} \sim D$ and then for each sample $x_i$, we take a sample $z$ with probability proportional to $p(x_i,z)(1\pm\delta)$ using Lemma \ref{lemma:sampling_runtime} and let our estimator $\hat{l} = \frac{1}{M}\sum_i|y_i-y|$. It is easy to see that this procedure requires $M = O(\frac{1}{\epsilon^2})$ label queries by construction and the total running time is $O(\frac{1}{\epsilon^2}*(\frac{d\log(N)^4}{\delta^2})\log(\frac{1}{\epsilon^2p}) = O(\frac{d\log(N)^4}{\epsilon^2\delta^2})\log(\frac{1}{\epsilon^2p})$. 
Now, we will prove that this estimator is within $E_{x,y \sim D}\sum_i^Np(x_i,x)|y_i-y| \pm \epsilon$ with high probability. First computing the expectation of the estimator, we get that 
\begin{align*}
E[\hat{l}] &= \frac{1}{M}\sum_iE_{x_i\sim D, z\sim p(x_i,z)(1\pm\delta)}[|y_i-y|]\\
&= \frac{1}{M}\sum_iE_{x_i\sim D}[\sum_{j=1}^Np(x_i,x_j)(1\pm\delta)|y_i-y_j|]\\
&= E_{x\sim D}[\sum_{j=1}^Np(x,x_j)|y-y_j|]\pm\delta\\
\end{align*}
%
Now, computing the variance of this estimator, we get that
\begin{align*}
Var_{x_i\sim D, z\sim p(x_i,z)(1\pm\delta)}[|y_i-y|^2] &= E_{x_i\sim D}[\sum_{j=1}^Np(x_i,x_j)(1\pm\delta)|y_i-y_j|^2] - (E_{x_i\sim D}[\sum_{j=1}^Np(x_i,x_j)(1\pm\delta)|y_i-y_j|])^2\\
&\leq  E_{x_i\sim D}[\sum_{j=1}^Np(x_i,x_j)(1\pm\delta)|y_i-y_j|^2] \leq 1\pm\delta
\end{align*}

Therefore, $Var(\hat{l}) = \frac{1\pm\delta}{M}$ since we are averaging $M$ independent and random estimators each with variance upper bounded by $1$. 

Therefore for $M \geq \frac{8}{\epsilon^2}$, using Chebyshev inequality, we get that 
$Pr(|\hat{l}-E[\hat{l}]| \geq \epsilon) \leq \frac{Var(\hat{l})}{\epsilon^2} \leq \frac{1\pm\delta}{8} \leq \frac{1}{4}$.

Therefore, the total error is atmost $\delta+\epsilon$ with failure probability atmost $p+\frac{1}{4}$

\end{proof}
%
%
\begin{lemma}
\label{lemma:sampling_runtime}
For a given query point $x$, it is possible to sample a training point $z \in S$ with probability proportional to $p(x,z)(1\pm \delta)$ in running time $O(\frac{d\log(N)^4}{\delta^2})\log(\frac{1}{p})$ with failure probability atmost $p$. 
\end{lemma}

\begin{proof}
First assume that all the $N$ training points are arranged in a tree like data structure where at the top level there are all the $N$ points $I_1 = z_1, z_2, \cdots, z_N$, then in the next level, there are two nodes, each having half the points, one node having $I_{21} = z_1, z_2, \cdots, z_{\frac{N}{2}}$ and the other having the other half i.e. $I_{22} = z_{\frac{N}{2}+1}, z_{\frac{N}{2}+2}, \cdots, z_{N}$ and so on till we reach the leaf nodes each having one exactly data point. Now, to sample a datapoint $z$ for a query point $x$ proportional to $p(x,z)(1\pm\delta)$, we traverse the tree in the following way: using the algorithm in \cite{backurs2018efficient} also restated in this paper as Theorem \ref{thm:backurs2018efficient}, we estimate $S_{21} = \sum_{i:x_i\in I_{21}}K(x,x_i)$ upto multiplicative accuracy of $\delta'$ to obtain $S'_{21} = S_{21}(1\pm\delta')$ and $S_{22} = \sum_{i:x_i\in I_{22}}K(x,x_i)$ upto  multiplicative accuracy of $\delta'$ to obtain $S'_{22} = S_{22}(1\pm\delta')$ and then choose node $I_{21}$ or $I_{22}$ with probabilities proportional to $p_{21}'=\frac{S'_{21}}{S'_{21}+S'_{22}} = \frac{S_{21}(1\pm\delta')}{S_{21}(1\pm\delta')+S_{22}(1\pm\delta')} = \frac{S_{21}}{S_{21}+S_{22}}(1\pm\delta')$ and similarly, $p_{22}'=\frac{S'_{21}}{S'_{21}+S'_{22}} = \frac{S_{22}}{S_{21}+S_{22}}(1\pm\delta')$ respectively and then recurse on the children nodes of the chosen node. 

Correctness of Algorithm:

Here, we compute the probability of sampling a point $z$ for the query point $x$, let us assume that without loss of generality, the point $z$ lies in the first child node of every node and lies at level $L$ of this tree. Then the probability that $z$ is chosen is equal to product of the probabilities of choosing its parent nodes at each of the levels. Hence, the probability would be given by $p_{x,z}' = \frac{S_{21}(1\pm\delta)}{S_{21}+S_{22}}\frac{S_{31}(1\pm\delta)}{S_{31}+S_{32}}\cdots\frac{S_{L1}(1\pm\delta)}{S_{L,1}+S_{L,2}}$ 
Now note that $S_{i-1,1} = S_{i,1}+S_{i,2}$. Hence, we get that
$p_{x,z}' \approx \frac{S_{L1}(1\pm\delta)^L}{S_{11}} \approx  p_{x,z}(1\pm L\delta')\approx p_{x,z}(1\pm \delta)$

For $\delta' = \frac{\delta}{\log(N)}$, we get that $1\pm L\delta' \approx 1\pm \delta$ since for the binary tree constructed in this way, the depth of tree would be $O(\log(N))$. 

Running time of Algorithm:

For each query, at each level we have to estimate $\sum_iK(x,x_i)$ upto error $\delta' = \frac{\delta}{\log(N)}$ with failure probability $\frac{p}{\log(N)}$ and the time required would be $\log(N)\frac{d\log(N)^3}{\delta^2}\log(\frac{\log(N)}{p}) = O(\frac{d\log(N)^4}{\delta^2})\log(\frac{1}{p})$ and $O(\frac{Nd}{\epsilon^2}\log(\frac{N}{\delta}))$ preprocessing time. 

\end{proof}


==> highd-lipschitz-camera-ready.tex <==
\subsection{Problem Setup}
We recall the setting from the one dimensional case.
%
For any fixed $L>0$, let $\mathcal{F}_{L}$ be the class of $d$ dimensional functions supported on the domain $[0,1]^d$ with Lipschitz constant at most $L$, that is,
\begin{equation}
    \mathcal{F}_L = \{f:[0,1]^d\mapsto [0,1], \  |f(x)-f(y)|\leq L \|x-y\|_{\infty} \;  \forall x,y \in [0,1]^d\}.
\end{equation}
 Let $\epsilon$ be the error parameter. We will think of the dimension $d$ as constant with respect to $L$ and $\epsilon$.
%Let $\D$ be any distribution over $[0,1]^d\times[0,1]$ with $\D_x$ the corresponding marginal distribution over $[0,1]^d$. The prediction error of a function $f$ with respect to $\D$ and the optimal prediction error of the class $\Fl$ are given by
%\begin{equation*}
%    \errd(f) \defn E_{x,y \sim \mathcal{D}}|y-f(x)| \quad \text{and} \quad \errd(\Fl) \defn \min_{f \in \mathcal{F}_L}E_{x,y \sim \mathcal{D}}|y-f(x)|.
%\end{equation*}
%Also, let us denote the error of a function $f$ relative to another function $f'$ and function class $\Fl$ as
%\begin{equation}
%    \diffd(f, f')\defn \errd(f) -\errd(f') \quad \text{and} \quad \diffd(f, \Fl) \defn  \errd(f) - \errd(\Fl).
%\end{equation}
%We say that a function $f\in \Fl$ is $\epsilon$-optimal with respect to distribution $\D$ and the function class $\Fl$ if it satisfies $\diffd(f, \Fl) \leq \epsilon$. Let functions $f^*_{\D} \in \Fl$ and $\hat{f}_S \in \Fl$ be the minimizers of error with respect to the distribution and  empirical error on set $S$ defined as
%\begin{align}
%f^*_{\D} = \argmin_{f \in \Fl } %\E_{(x, y) \sim \D}|y-f(x)| \quad %\text{ and } \quad 
%\hat{f}_S = \argmin_{f \in \Fl } \sum_{(x_j, y_j) \in %S}|y_j-f(x_j)|,\label{lipschitz:minemperror}
%\end{align}% 
%
%
 %Let $\mathcal{F}_{L}$ be the class of  Lipschitz functions supported on the interval $[0,1]^d$ with Lipschitz constant at most $L$ where $d$ is the dimension that is any $f$ belonging to $\mathcal{F}_L$ satisfies $|f(x)-f(y)|\leq||x-y||_{\infty} \ \forall x,y \in [0,1]^d$. Let $\epsilon$ be the accuracy parameter. We will think of the dimension $d$ as constant with respect to $L$ and $\epsilon$. We are interested in locally predicting the label for any query $x$ such that labeled sample complexity is independent of $L$ corresponding to a function in the class $\mathcal{F}_{L}$ which is nearly optimal. 
Like the one-dimensional case, our algorithm for local predictions first involves a preprocessing step (Algorithm~\ref{alg4}) 
which takes as input the Lipschitz constant $L$, sampling access to distribution $\D_x$ and the error parameter $\epsilon$ and returns a partition $\p$ where the partition along dimension $j$ is $\p^j = \{ [b^j_0, b^j_1],[b^j_1, b^j_2], \ldots, \}$ and a set $S$ of unlabeled samples. The partition $\p$ consists of alternating intervals\footnote{Note that long intervals at the boundary could be shorter, but those can be handled similarly. } of length ${2}/{L}$ and ${d}/(L\epsilon)$ along each dimension. Let us divide these intervals along each dimension $j$ further into the two sets 
\begin{equation*}
    \begin{gathered}
    \plong^j\defn\{[b_0,b_1],[b_2,b_3],\ldots,\}\quad \text{(long intervals for dimension } j \text{ of length } {d}/(L\epsilon)), \\
    \pshort^j\defn\{[b_1,b_2],[b_3,b_4],\ldots,\}\quad \text{(short intervals for dimension } j \text{ of length }{2}/L).\\
    \end{gathered}
\end{equation*}


%The longer intervals of length ${d}/(L\epsilon)$ along each dimension are labeled as type 1 intervals for that dimension whereas the shorter intervals of length ${2}/{L}$ are labeled as type 2 intervals for that dimension. 
A data point $x$ which belongs to a short interval in $\p^j$ along at least one of the dimensions $j$ is said to belong to a set of short intervals $\pshort$ and otherwise, is said to belong to a set of long intervals $\plong$.
% 
% 
 \begin{algorithm}[H]
   \begin{algorithmic}[1]
\caption{Preprocess($L, \D_x, \epsilon$)\label{alg4}}
   \STATE Sample a uniformly random offset $b^j_1$ from $\{0,1,2,\cdots,\frac{d}{2\epsilon}\}\frac{2}{L}$ for each dimension $j \in [d]$. 
   \STATE Divide the $[0,1]$  interval along each dimension $j$ into alternating intervals of length $\frac{d}{L\epsilon}$ and $\frac{2}{L}$ with boundary at $b^j_1$ and let $\p$ be the resulting partition, that is, $\p^j = \{[b^j_0=0,b^j_1],[b^j_1, b^j_2], \ldots, ], \cdots, 1\}$ where $b^j_2 = b^j_1 + \frac{2}{L}, b_3^j = b_2^j + \frac{d}{L\epsilon}, \ldots, $. 
%   \STATE The intervals $\{[b^i_1,b^i_2],[b^i_3,b^i_4],\cdots,\}$ are called type 2 intervals for dimension $i$. Any $x \in [0,1]^d$ which has at least one coordinate $x_i\in\{[b^i_1,b^i_2],[b^i_3,b^i_4],\cdots,\}$ will be said to belong to a type 2 interval.\\
   \STATE Sample a set $S = \{x_i\}_{i=1}^M$ of $M = O((\frac{L}{\epsilon})^d \frac{1}{\epsilon^3}\log(\frac{1}{\epsilon}))$ unlabeled examples from distribution $\mathcal{D}_x$.\\
   \STATE \textbf{Output} $S, \p$.
   %\vspace{1.783cm}
   \end{algorithmic}
  \end{algorithm}
%
%
%
%
We give the definition of the extension interval for a long interval in $\plong$. It consists of a long interval and a cuboidal shell of thickness $\frac{1}{L}$ around it in each dimension and cut off at the boundary.
%
%
\begin{definition}
\label{defn:extension-interval}
For any long interval $I_J$ where $I_J^i=[b^i_{J^i-1}, b^i_{J^i}]$, the extension interval is defined to be $\hat{I}_J$ where $\hat{I}_J^i = [\max(0,b^i_{J^i-1}-\frac{1}{L}),\min(b^i_{J^i}+\frac{1}{L},1)]$ $\forall i \in [d]$ such that $I_J \subset \hat{I}_J$. In other words, interval $\hat{I}_J$ consists of the interval $I_J$ and a cuboidal shell of thickness $\frac{1}{L}$ around it on both sides in each dimension unless it does not extend beyond $[0,1]$ in each dimension.
\end{definition}
%
%
The Query algorithm (Algorithm~\ref{alg5}) for test point $x^*$ takes as input the set $S$ of unlabeled examples and the partition $\p$ returned by the Preprocess algorithm. Note that all subsequent queries use the same partition $\p$ and the same set of unlabeled examples $S$. The algorithm uses different learning strategies depending on whether $x^*$ belongs to one of the long intervals in $\plong$ or short intervals in $\pshort$.

For the long intervals, it outputs the prediction corresponding to the empirical risk minimizer (ERM) function restricted to that interval. The middle function values of the short intervals are constrained to be $1$ which makes the overall function Lipschitz. If a query point $x$ lies in a short interval which is the Lipschitz extension of a given long interval, the function learned is the Lipschitz extension of function over the long interval. This ensures that the overall function is Lipschitz. We bound the expected prediction error of this scheme with respect to class $\Fl$ by separately bounding this error for long and short intervals. For the long intervals, we prove that the ERM has low error by ensuring that each interval contains enough unlabeled samples. On the other hand, we show that the short intervals do not contribute much to the error because of their low probability under the distribution $\D$.
%
%
%
 \begin{algorithm}[H]
   \begin{algorithmic}[1]
\caption{Query($x, S, \p=[\{[b^j_0,b^j_1],[b^j_1, b^j_2],\cdots\}]^d_{j=1}$)\label{alg5}}
    %\STATE S, P = Preprocess(L)
   \IF{query $x \in I_J \text{ where } I^j_J = [b^j_{J^j-1}, b^j_{J^j}] \text{ when } I_J \in \plong$ }
   %
     \STATE Query labels for $x \in S \cap I_J$
   \STATE \textbf{Output} $\hat{f}_{S \cap I_J}(x)$ \\

    \ELSIF{query $x \in \hat{I}_J$ where  $\hat{I}_J$ is the extension of a long interval $I_J$ where $I^j_J = [b^j_{J^j-1}, b^j_{J^j}]$ is a long interval}
    %
     \STATE Query labels for $x \in S \cap I_J$
   \STATE \textbf{Output:} $f(x)$ where $f(x)$ is the Lipschitz extension of $f_J(x)$ to the extension set $\hat{I}_{J}$ with constraints $f(x) = 1$ $\forall x \in \hat{I}_{J}$ satisfying $x_i \in \Big\{\frac{b^i_{J^i}+b^i_{J^i+1}}{2},\frac{b^i_{J^i-2}+b^i_{J^i-1}}{2}\Big\}$ for at least one $i \in [d]$. 
    %
\ELSE
    \STATE \textbf{Output:} 1
%
    %
\ENDIF
   %\vspace{1.783cm}
   \end{algorithmic}
  \end{algorithm}
%
%
Next, we state the number of label queries needed to making local predictions corresponding to the Query algorithm (Algorithm \ref{alg5}).
%
%
\begin{theorem}
\label{thm:lipschitzlocalquery-highd}
For any distribution $\mathcal{D}$ over $[0,1]^d\times[0,1]$, Lipschitz constant $L>0$ and error parameter $\epsilon \in [0,1]$, let $(S, P)$ be the output of (randomized) Algorithm~\ref{alg1} where $S$ is the set of unlabeled samples of size $(O(\frac{L}{\epsilon}))^d\frac{1}{\epsilon^3}\log(\frac{1}{\epsilon})$ and $P$ is a partition of the domain $[0,1]^d$. Then, there exists a function  $\tilde{f} \in \mathcal{F}_L$, such that for all $x \in [0,1]$, Algorithm~\ref{alg5} queries $\frac{1}{\epsilon^2}(O(\frac{d}{\epsilon^2}))^d\log(\frac{1}{\epsilon})$ labels from the set $S$ and outputs $\text{Query}(x, S, P) $ satisfying
\begin{equation}
    \text{Query}(x, S, P) = \tilde{f}(x)\;,
\end{equation}
and the function $\tilde{f}$ is $\epsilon$-optimal, that is, $ \diffd(\ft, \Fl) \leq \epsilon$ with probability greater than $\frac{1}{2}$.
%\begin{equation}
%    |E_{x,y \sim \mathcal{D}}|y-\tilde{f}(x)| - \min_{f \in \mathcal{F}_L}E_{x,y \sim \mathcal{D}}|y-f(x)|| \leq \epsilon,
%\end{equation}
\end{theorem}
\iffalse
\begin{theorem}
\label{thm:lipschitzlocalquery-highd}
Let data points $(x,y) \sim \mathcal{D}$ and let $\mathcal{F}_L$ be the class of Lipschitz functions with Lipschitz constant at most $L$. Then, there exists a $L$ Lipschitz function $\tilde{f}(x):[0,1]^d \rightarrow [0,1]$ such that $|E_{x,y \sim \mathcal{D}}|y-\tilde{f}(x)| - \min_{f \in \mathcal{F}_L}E_{x,y \sim \mathcal{D}}|y-f(x)|| \leq \epsilon$ and for a fixed given $x \in [0,1]^d$, $\tilde{f}(x)$ can be computed with $(O(\frac{L}{\epsilon}))^d\frac{1}{\epsilon^3}$ unlabeled samples $x,y \sim \mathcal{D}$ and $\frac{1}{\epsilon^2}(O(\frac{d}{\epsilon^2}))^d$ active label queries on those unlabeled samples.
\end{theorem}
\fi
%
\begin{proof}
 We begin by defining some notation. Let $S= \{x_i\}^M_{i=1}$ be the set of the unlabeled samples and $\p=\{[b_0,b_1],[b_1,b_2], \ldots\}$ be the partition returned by the pre-processing step given by Algorithm~\ref{alg5}. 
%
Let $\D_J$ be the distribution of a random variable  $(X, Y) \sim \D$ conditioned on the event $\{X \in I_J\}$. Similarly, let $\Dsh$ and $\Dlg$ be the conditional distribution of $\D$ on intervals belonging to $\plong$ and $\pshort$ respectively. Let $p_J$ denote the probability of a point sampled from distribution $\D$ lying in interval $I_J$. Going forward, we use the shorthand `probability of interval $I_J$' to denote $p_J$. Let $\plg$ and $\psh$ be the probability of set of long and short intervals respectively. Recall that $f_{\D}^*$ is the function which minimizes $\errd(f)$ for $f \in \Fl$ and $f_{\D_J}^*$ is the function which minimizes this error with respect to the conditional distribution $\D_J$. Let $M_J$ denote the number of unlabeled samples of $S$ lying in interval $I_J$. For any interval $I_J$, let $\hat{f}_{S\cap I_J}$ be the ERM with respect to that interval.%
%
\paragraph{Lipschitzness of $\ft$.} For $x$ belonging to intervals say $I_J$ where $I^j_J= [b^j_{J^j-1}, b^j_{J^j}], j\in [d]$ where $I_J \in \pshort$, let $f_J(x)$ be defined by the output of the Algorithm~\ref{alg5}. Now, let $\tilde{f}:[0,1]^d\rightarrow[0,1] = f_J(x) \text{ if } x \in I_J$ be disjoint union of the functions $f_J$ defined on disjoint intervals $I_J$. Now, we will argue that $\tilde{f}(x)$ is $L$ Lipschitz for all $x\in[0,1]^d$. The function $\tilde{f}(x)$ for each long interval is $L$ Lipschitz by construction. For each long interval $I_J$ where $I^j_J = [b^j_{J^j-1},b^j_{J^j}]$ $\forall j \in [d]$, consider the extension interval $\hat{I}_J$ as defined in Definition~\ref{defn:extension-interval}. The function $\tilde{f}(x)$ is constrained to be $1$ for the middle point of the short interval along each dimension i.e. $\tilde{f}(x) = 1$ $\forall x\in[0,1]^d\text{ if } \exists i\in[d] \text{ such that }x_i=\frac{b^i_{j-1}+b^i_{j}}{2}$ where $[b^i_{j-1},b^i_{j}]$ is a short interval for dimension $i$. Note that these middle points of short intervals are precisely the only points of intersection between extensions of two different long intervals because long intervals in each dimension are separated by a distance of $\frac{2}{L}$ by construction and the extension intervals extend up to a shell of thickness around $\frac{1}{L}$ in each dimension. Now, for a query point $x$ belonging to extension interval $\hat{I}_J$ for a long interval $I_J$ takes the value $f(x)$ where $f(x)$ is the Lipschitz extension of the Lipschitz function $f_J$ to the superset $\hat{I}_J$ and constrained to be $1$ at the boundary of the shell. Hence, if we can prove that such a Lipschitz extension exists, we can see that the combined function is $L$ Lipschitz. By \cite{mcshane1934extension} (also stated as Theorem~\ref{thm:lipschitz-extension} in this paper), we can see that such a Lipschitz extension always exists because for point $x \in I_J$ and $y$ belonging to the boundary of the shell, we get that $||x-y||_{\infty} \geq \frac{1}{L}$ and $|f(x)-f(y)|\leq 1$ and hence, the function $f$ is $L$-Lipschitz. For query points $x$ which do not belong to any of these extension intervals, we output $1$. Basically, these points belong to the short intervals at the boundary of the domain and equivalent to learning Lipschitz extension with empty long interval and constrained to be $1$ at the boundary. Hence, the function takes $1$ everywhere in this interval. Hence, we can see that the function $\tilde{f}$ is $L$-Lipschitz. 
%
%
\paragraph{Error Guarantees for $\ft$.} Now looking at the error rate of the function $\tilde{f}(x)$ and following a repeated application of tower property of expectation, we get that 
%
%
\begin{align}
    \diffd(\ft, \Fl) &= \plg\diff_{\Dlg}(\ft, f_{\D}^*) + \psh\diff_{\Dsh}(\ft, f_{\D}^*)\nonumber\\
    &= \sum_{J:I_J \in \plong}p_J\diff_{\D_J}(\ft, f_{\D}^*) + \psh\diff_{\Dsh}(\ft, f_{\D}^*)\label{eqn:total-error-highd}
\end{align}
%
Now, we need to argue about the error bounds for both long and short intervals to argue about the total error of the function $\tilde{f}$.

\emph{Error for short intervals. } 
%
The probability of short intervals $\psh$ is small with high probability since the total length of short intervals is $2\epsilon$ and the intervals are chosen uniformly randomly. More formally, from Lemma~\ref{lemma:prob_intervals-highd}, we know that with probability at least $1-\delta$, the probability of short intervals $\psh$ is upper bounded by $2\epsilon/\delta$. Also, the error for any function $f$ is bounded between $[0,1]$ since the function's range is $[0,1]$. Hence, we get that
%
\begin{align}
\psh\diff_{\D_{\pshort}}(\ft, f_{\D}^*) &\leq \frac{2\epsilon}{\delta} \label{eqn:type2-error-highd}
\end{align}
%
%
\emph{Error for long intervals:} We further divide the long intervals into 3 subtypes: 
{\small
\begin{align*}
    %\begin{gathered}
    \plongone &\defn \left\lbrace I_J \; |\; I_J \in \plong,\; p_J \geq\frac{\epsilon}{(\frac{L\epsilon}{d})^d},\; M_J \geq  \frac{1}{\epsilon^2}(\Omega(\frac{d}{\epsilon^2}))^d)\log(\frac{1}{\epsilon}) \right\rbrace,\\ %\quad
    \plongtwo &\defn \left\lbrace I_J \; |\; I_J \in \plong,\; p_J \geq\frac{\epsilon}{(\frac{L\epsilon}{d})^d},\; M_J <  \frac{1}{\epsilon^2}(\Omega(\frac{d}{\epsilon^2}))^d)\log(\frac{1}{\epsilon}) \right\rbrace,\\ 
   \plongthree &\defn \left\lbrace I_J \; |\; I_J \in \plong,\; p_J < \frac{\epsilon}{(\frac{L\epsilon}{d})^d} \right\rbrace.
    %\end{gathered}
\end{align*}}
The intervals in both first and second types have large probability $p_J$ with respect to distribution $\D$ but differ in the number of unlabeled samples in $S$ lying in them. Finally, the intervals in third subtype $\plongthree$ have small probability $p_J$ with respect to distribution $\D$. Now, we can divide the total error of long intervals into error in these subtypes
%
%
\begin{small}
\begin{align}
\sum_{J:I_J \in \plong}p_J\diff_{\D_J}(\ft, f_{\D}^*) &= \underbrace{\sum_{J:I_J \in \plongone}p_J\diff_{\D_J}(\ft, f_{\D}^*)}_{E1} + \underbrace{\sum_{J:I_J \in \plongtwo}p_J\diff_{\D_J}(\ft, f_{\D}^*)}_{E2}+ \underbrace{\sum_{J:I_J \in \plongthree}p_J\diff_{\D_J}(\ft, f_{\D}^*)}_{E3} 
\label{eqn:combined-highd}
\end{align}
\end{small}
%
%
Now, we will argue about the contribution of each of the three terms above. 

\underline{Bounding $E3$.} Since there are at most $(\frac{L\epsilon}{d})^d$ long intervals and each of these intervals $I_J$ has probability $p_J$ upper bounded by $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$, the total probability combined in these intervals is at most $\epsilon$. Also, in the worst case, the loss can be 1. Hence, we get an upper bound of $\epsilon$ on $E_3$.
%

\underline{Bounding $E2$.} From Lemma~\ref{lemma:number_unlabeled_samples-highd}, we know that with success probability $\delta$, these intervals have total probability upper bounded by ${\epsilon}/{\delta}$. Again, the loss can be 1 in the worst case. Hence, we can get an upper bound of ${\epsilon}/{\delta}$ on $E_2$.

\underline{Bounding $E1$.}  
%
%
Let $F_J$ denote the event that $\diff_{\D_J}(\hat{f} _{S\cap I_J}, f_{\D_J}^*) > \epsilon$.  The expected error of intervals $I_J$ in $\plongone$ is then
{\small
\begin{align*}
\E[\sum_{J:I_J \in \plongone}p_J\diff_{\D}(\ft, f_{\D_J}^*)] &\stackrel{\1}{\leq} \E[\sum_{J:I_J \in \plongone}p_J\diff_{\D_J}(\hat{f}_{S\cap I_J}, f_{\D_J}^*)]\\ 
%&\stackrel{\2}{=} \E[\sum_{i:I_i \in \plongone}p_i\diff_{\D_i}(\hat{f}_i, f_i^*)]\\ 
&= \sum_{J:I_J \in \plongone}p_J(\E[\diff_{\D_J}(\hat{f}_{S\cap I_J}, f_{\D_J}^*)|F_J]\Pr(F_J) + \E[\diff_{\D_J}(\hat{f}_{S\cap I_J}, f_{\D_J}^*)|\neg F_J]\Pr(\neg F_J))\\
%
&\stackrel{\2}{\leq} \sum_{J:I_J \in \plongone}p_J(1\cdot \epsilon + \epsilon \cdot 1) 
\leq 2\epsilon,
\end{align*}}
%
%
%
where step $\1$ follows by noting that $\ft = \hat{f}_{S\cap I_J}$ for all long intervals $I_J \in \plong$ and that $f^*_{\D_J}(x)$ is the minimizer of the error $\err_{\D_J}(f)$ over all $L$-Lipschitz functions, 
%$$E_{x,y\sim \mathcal{D}_i}|f^*_i(x) - y| \leq E_{x,y\sim \mathcal{D}_i}|f^*(x) - y| \quad \forall I_i \in \plongone$$
and step $\2$ follows since $\E[\diff_{\D_J}(\hat{f}_{S\cap I_J}, f_{\D_J}^*)|\neg F_J] \leq \epsilon$ by the definition of event $F_J$ and $\Pr(F_J) \leq \epsilon$ follows from a standard uniform convergence argument (detailed in Lemma~\ref{lem: good type 1 intervals-highd}).
Now, using Markov's inequality, we get that $E_1 \leq {2\epsilon}/{\delta}$ with failure probability at most $\delta$. 

Plugging the error bounds obtained in equations~\eqref{eqn:type2-error-highd} and ~\eqref{eqn:combined-highd} into equation~\eqref{eqn:total-error-highd} and setting $\delta = \frac{1}{20}$ establishes the required claim.

%
%
\paragraph{Label Query Complexity.} Observe that for any given query point $x^*$, $\ft(x^*)$ can be computed by only querying the labels of the interval in which $x$ lies (in case if $x^*$ lies in a long interval) or extension of the interval in which $x^*$ lies (in case if $x^*$ lies in a short interval) and hence, would only require $\frac{1}{\epsilon^2}(O(\frac{d}{\epsilon^2}))^d\log(\frac{1}{\epsilon})$ active label queries over the set $S$ of $\frac{1}{\epsilon^3}(O(\frac{L}{\epsilon}))^d\log(\frac{1}{\epsilon})$ unlabeled samples.
%   
\end{proof}
%
%
Now, we will state the sample complexity bounds for estimating the error of the optimal function amongst the class of Lipschitz functions up to an additive error of $\epsilon$. 
%
\begin{restatable}{theorem}{theoremlipschitzerror-highd}
%\begin{theorem}
\label{thm:lipschitzerror-highd}
For any distribution $\mathcal{D}$ over $[0,1]^d\times[0,1]$, Lipschitz constant $L>0$ and parameter $\epsilon \in [0,1]$, Algorithm~\ref{alg3} uses $\frac{1}{\epsilon^4}(O(\frac{d}{\epsilon^2}))^d\log(\frac{1}{\epsilon})$ active label queries on $\frac{1}{\epsilon^3}(O(\frac{L}{\epsilon}))^d\log(\frac{1}{\epsilon})$ unlabeled samples from distribution $\D_x$ and produces an output $\widehat{\errd}(\Fl)$ satisfying
\begin{equation*}
|\widehat{\errd}(\Fl) - \errd( \Fl)| \leq \epsilon 
\end{equation*} 
with probability at least $\frac{1}{2}$.
%\end{theorem}
\end{restatable}
%
%\begin{restatable}{theorem}{theoremlipschitzerrorhighd}
%\begin{theorem}
%\label{thm:lipschitzerror-highd}
%For data points $(x,y)\in([0,1]^d\times[0,1])$ drawn from distribution $\mathcal{D}$ and the class of $L$-Lipschitz functions $\mathcal{F}_L$, it is possible to estimate $\min_{f \in \mathcal{F}_L}E_{x,y \sim \mathcal{D}}|y-f(x)|$ up to an additive error $\epsilon$ with $O(\frac{1}{\epsilon^4}(O(\frac{d}{\epsilon^2}))^d)$ active label queries on $\frac{1}{\epsilon^3}(O(\frac{L}{\epsilon}))^d$ unlabeled samples randomly sampled from distribution $\mathcal{D}$ and an additional $O(\frac{1}{\epsilon^2})$ labeled samples from distribution $\mathcal{D}$.
%\end{theorem}
%\end{restatable}
%
The proof goes exactly like the proof for the corresponding theorem in the one-dimensional case (Theorem~\ref{thm:lipschitzerror}).
%

The following lemma proves that with enough unlabeled samples, a large fraction of long intervals have enough unlabeled samples in them which is eventually used to argue that they will be sufficient to learn a function which is approximately close to the optimal Lipschitz function over that interval. 
%
\begin{lemma}
\label{lemma:number_unlabeled_samples-highd}
For any distribution $\D_x$, consider a set $S = \{x_1, x_2, \cdots, x_M\}$ of unlabeled samples where each sample $x_i\stackrel{\text{i.i.d.}}{\sim}\D_x$. Let $\mathcal{G}$ be the set of long intervals $\{I_i\}$ each of which satisfies $p_J = \Pr_{x \sim \D_x}(x \in I_J) \geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$. Let $E_J$ denote the event that $\sum_{x_j \in S}\mathbb{I}[x_j \in I_J] < \frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d\log(\frac{1}{\epsilon})$. Then, we have 
\begin{equation*}
    \sum_{I_J \in \mathcal{G}}p_J\mathbb{I}[E_J] \leq \frac{\epsilon}{\delta}
\end{equation*}
with failure probability atmost $\delta$ for $M = \frac{1}{\epsilon^3}(\Omega(\frac{L}{\epsilon}))^d\log(\frac{1}{\epsilon})$. 
\end{lemma}
%

\begin{proof}
For any interval $I \in \mathcal{G}$, we have that $\E[\sum_{x_j \in S}\mathbb{I}[x_j \in I]] \geq \frac{c_d}{\epsilon^2}(\frac{d}{\epsilon^2})^d\log(\frac{1}{\epsilon})$ for some constant $c_d$ depending on the dimension $d$. Using Hoeffding inequality, we can get that $\Pr(E_i) \leq \epsilon$ for all intervals $I_i \in \mathcal{G}$. Calculating expectation of the desired quantity, we get
\begin{equation*}
    \E[\sum_{I_J \in \mathcal{G}}p_J\mathbb{I}[E_J]] = \sum_{I_J \in \mathcal{G}}p_J\Pr[E_J] \leq \epsilon\sum_{I_J \in \mathcal{G}}p_J \leq \epsilon
\end{equation*}

%
We get the desired result using Markov's inequality.
\end{proof}

%
%
\iffalse
\begin{proof}
The expected number of samples that falls in an interval $I$ will probability mass greater than $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ is at least $\frac{c_d}{\epsilon^2}(\frac{d}{\epsilon^2})^d$ for some constant $c_d$ depending on the dimension $d$. Using Chernoff bounds, we can get that $Pr(\text{number of samples in } I \leq \frac{c_d}{2\epsilon^2}(\frac{d}{\epsilon^2})^d) \leq \exp(-\frac{c_dd^d}{8\epsilon^{2(d+1)}}) \leq \epsilon$. Now, let $F_i$ be the event that $I_i$ interval which has probability mass $\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ has $\leq \frac{c_d}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples in it. Now, we know that $F_i \leq \epsilon$ $\forall i$ where $I_i$ is an interval of type 1 having probability mass greater than $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$. Now, the expected combined mass of type 1 intervals which have $\leq \frac{c_d}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples is $\sum_iPr(F_i)Pr(I_i) \leq \epsilon\sum_iPr(I_i) \leq \epsilon$. Now, using Markov's inequality, we get that with probability at least $1-\delta$, the total mass of type 1 intervals having $\leq \frac{c_d}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples each is $\leq \frac{\epsilon}{\delta}$.  
\end{proof}
\fi
%
%
%
The following lemma states that the probability of short intervals $\psh$ is small with high probability. Consider the case of uniform distribution. In this case, since the short intervals cover only $2\epsilon$ fraction of the domain $[0,1]^d$, their probability $\psh$ is upper bounded by $2\epsilon$. The case for arbitrary distributions holds because the intervals are chosen randomly.
%
%
\begin{lemma}
\label{lemma:prob_intervals-highd}
When we divide the $[0,1]^d$ domain into long and short intervals as in the preprocessing step (Algorithm~\ref{alg4}), then
\begin{equation*}
    \psh = \sum_{I_J \in \pshort}p_J \leq \frac{2\epsilon}{\delta}
\end{equation*}
with failure probability atmost $\delta$. 
\end{lemma}
%
%
\iffalse
\begin{lemma}
\label{lemma:prob_intervals-highd}
When we divide the $[0,1]^d$ domain into type 1 and type 2 intervals as in the preprocessing step \ref{alg4}, then with probability more than $1-\delta$, a randomly sampled $x\sim \mathcal{D}$ lies in intervals of type 1 or type 2 intervals have probability mass bounded by $\frac{2\epsilon}{\delta}$ with probability $1-\delta$.
\end{lemma}
\fi
%
\begin{proof}
Now, we consider the division of every dimension i.e. $[0,1]$ independently into alternating intervals of length $\frac{d}{L\epsilon}$ and $\frac{2}{L}$ with the offset chosen uniformly randomly from $\{0, 1, 2, \cdots, \frac{d}{2\epsilon}\}\frac{2}{L}$. For any set of fixed offsets chosen for the $d-1$ dimensions, the intervals of length $\frac{2}{L}$ chosen for the $dth$ dimension combined are disjoint in each of these divisions and together cover the entire $[0,1]^d$ and hence amount to probability mass $1$. Therefore, the total probability mass covered in the total $(\frac{d}{2\epsilon}+1)^d$ possible divisions is $d(\frac{d}{2\epsilon}+1)^{d-1}$.  Hence, there are at most $\delta$ fraction out of the total $(\frac{d}{2\epsilon}+1)^d$ cases where the short intervals have probability greater than $\frac{2\epsilon}{\delta}$. Hence, with probability $1-\delta$, the short intervals have probability upper bounded by $\frac{2\epsilon}{\delta}$. %
\end{proof}

\begin{lemma}
\label{lem: good type 1 intervals-highd}
Let $I_i \in \plongone$ be any long interval of subtype 1. For the event \mbox{$F_i = \{\diff_{\D_i}(\hat{f}_{S \cap I_i}, f_{\D_i}^*) > \epsilon
\}$}, we have
\begin{equation*}
    \Pr(F_i) \leq \epsilon
\end{equation*}
\end{lemma}

\begin{proof}
We know that the covering number for the class of $d$-dimensional $L$-Lipschitz functions supported on the interval $[0,l]$ is $(O({Ll}/{\epsilon}))^d$ (Lemma~\ref{lemma:lipschitz_covering}). For, Lipschitz functions supported on long intervals of length $l={d}/{(L\epsilon)}$ along each dimension, we get this complexity as $(O({d}/{\epsilon^2}))^d$.  We know by standard results in uniform convergence, that the number of samples required for uniform convergence up to an error of $\epsilon$ and failure probability $\delta$ for all functions in a class $\mathcal{F}_L$ is $\Omega(((\text{Covering number of } \mathcal{F}_L)/\epsilon^2)\log({1}/{\delta}))$ (Lemma~\ref{lemma:lipschitz_sample_complexity}) and hence, for long intervals we get this estimate as $\frac{1}{\epsilon^2}(\Omega(\frac{d}{\epsilon^2}))^d\log(\frac{1}{\delta})$. 
Given that there are $\frac{1}{\epsilon^2}(\Omega(\frac{d}{\epsilon^2}))^d\log(\frac{1}{\epsilon})$ samples in these intervals by design, the function learned using these samples is only additively worse than the function with minimum error using standard learning theory arguments with failure probability at most $\epsilon$. Thus, we get that 
$$\diff_{\D_i}(f_{S \cap I_i}, f_{\D_i}^*) \leq \epsilon \quad \forall I_i \in \plongone$$
with failure probability at most $\epsilon$. 
\end{proof}

==> new-highd.tex <==
\begin{theorem}
\label{thm:lipschitzlocalquery}
For any distribution $\mathcal{D}$ over $[0,1]\times[0,1]$, Lipschitz constant $L>0$ and error parameter $\epsilon \in [0,1]$, let $(S, P)$ be the output of (randomized) Algorithm~\ref{alg1} where $S$ is the set of unlabeled samples of size $O(\frac{L}{\epsilon^4}\log(\frac{1}{\epsilon}))$ and $P$ is a partition of the domain $[0,1]$. Then, there exists a function  $\tilde{f} \in \mathcal{F}_L$, such that for all $x \in [0,1]$, Algorithm~\ref{alg2} queries $O(\frac{1}{\epsilon^4}\log(\frac{1}{\epsilon}))$ labels from the set $S$ and outputs $\text{Query}(x, S, P) $ satisfying
\begin{equation}
    \text{Query}(x, S, P) = \tilde{f}(x)\;,
\end{equation}
and the function $\tilde{f}$ is $\epsilon$-optimal, that is, $ \diffd(\ft, \Fl) \leq \epsilon$ with probability greater than $\frac{1}{2}$.
%\begin{equation}
%    |E_{x,y \sim \mathcal{D}}|y-\tilde{f}(x)| - \min_{f \in \mathcal{F}_L}E_{x,y \sim \mathcal{D}}|y-f(x)|| \leq \epsilon,
%\end{equation}
\end{theorem}
\begin{proof}
%
%
%
%
\paragraph{Lipschitzness of $\ft$.}
For any interval $I_i = [b_{i-1}, b_i]$, let $v_i^l = \hat{f}_{S\cap I_{i-1}}(b_{i-1})$ be the value of the function with minimum empirical error on the neighbouring interval $I_{i-1}$ at the boundary point $b_{i-1}$  and similarly $v_i^u = \hat{f}_{S\cap I_{i+1}}(b_{i})$ is the value of the function $\hat{f}_{S\cap I_{i+1}}$ at the boundary point $b_i$. Note that if $I_i$ is a boundary interval and therefor $I_{i-1}$ (or $I_{i+1}$) does not exist, we can define $v^l_i=v^u_i$ (or $v^u_i=v^l_i$).
Further, let $f^{\sf{int}}_i: I_i \mapsto \R$ be the linear function interpolating from $v_i^l$ to $v_i^u$, that is, 
\begin{equation*}
 f^{\sf{int}}_i(x) = v^l_i+(x-b_{i-1})\frac{v_i^l-v^u_i}{b_i-b_{i-1}}.
\end{equation*}
Note that the Query procedure (Algorithm~\ref{alg2}) is designed to output $\ft(x)$ for each query $x$ where
\begin{equation*}
       \ft(x) = \begin{cases}
       \hat{f}_{S\cap I_i}(x) \quad &\text{ if } x \in I_i \text{ for any } I_i \in \plong\\
        f^{\sf{int}}_i(x) \quad &\text{ if } x \in I_i \text{ for any } I_i \in  \pshort
       \end{cases}.
\end{equation*}
Now, it is easy to see that the function $\ft(x)$ is $L$-Lipschitz. The function $\hat{f}_{S\cap I_i}$ on each of the long intervals is $L$-Lipschitz by construction. The function ${f_i^{\sf{int}}}$ on each of the short intervals is also $L$-Lipschitz since the short intervals in $\pshort$ have length ${1}/{L}$ and the label values  $y_j \in [0,1]$. Also, the function $\ft$ is continuous at the boundary of each interval by construction. 
%
\paragraph{Error Guarantees for $\ft$.}
%
%
%

\emph{Error for long intervals:} 
%
%
%
%
%
%

\underline{Bounding $E1$.}  
%
%
Let $F_i$ denote the event that $\diff_{\D_i}(\hat{f} _{S\cap I_i}, f_{\D_i}^*) > \epsilon$.  The expected error of intervals $I_i$ in $\plongone$ is then
{\small
\begin{align*}
\E[\sum_{i:I_i \in \plongone}p_i\diff_{\D}(\ft, f_{\D_i}^*)] &\stackrel{\1}{\leq} \E[\sum_{i:I_i \in \plongone}p_i\diff_{\D_i}(\hat{f}_{S\cap I_i}, f_{\D_i}^*)]\\ 
%&\stackrel{\2}{=} \E[\sum_{i:I_i \in \plongone}p_i\diff_{\D_i}(\hat{f}_i, f_i^*)]\\ 
&= \sum_{i:I_i \in \plongone}p_i(\E[\diff_{\D_i}(\hat{f}_{S\cap I_i}, f_{\D_i}^*)|F_i]Pr(F_i) + \E[\diff_{\D_i}(\hat{f}_{S\cap I_i}, f_{\D_i}^*)|\neg F_i]Pr(\neg F_i))\\
&\stackrel{\2}{\leq} \sum_{i:I_i \in \plongone}p_i(1\cdot \epsilon + \epsilon \cdot 1) 
\leq 2\epsilon,
\end{align*}}
%
%
%
where step $\1$ follows by noting that $\ft = \hat{f}_{S\cap I_i}$ for all long intervals $I_i \in \plong$ and that $f^*_{\D_i}(x)$ is the minimizer of the error $\err_{\D_i}(f)$ over all $L$-Lipschitz functions, 
%$$E_{x,y\sim \mathcal{D}_i}|f^*_i(x) - y| \leq E_{x,y\sim \mathcal{D}_i}|f^*(x) - y| \quad \forall I_i \in \plongone$$
and step $\2$ follows since $\E[\diff_{\D_i}(\hat{f}_{S\cap I_i}, f_{\D_i}^*)|\neg F_i] \leq \epsilon$ by the definition of event $F_i$ and $\Pr(F_i) \leq \epsilon$ follows from a standard uniform convergence argument (detailed in Lemma~\ref{lem: good type 1 intervals}).
Now, using Markov's inequality, we get that $E_1 \leq {2\epsilon}/{\delta}$ with failure probability at most $\delta$. 

Plugging the error bounds obtained in equations~\eqref{eqn:type2-error} and ~\eqref{eqn:combined} into equation~\eqref{eqn:total-error} and setting $\delta = \frac{1}{10}$ establishes the required claim.


\end{proof}

==> oldhighd-lipschitz.tex <==
%
 \begin{algorithm}[H]
   \begin{algorithmic}[1]
\caption{Preprocess(L)\label{alg1-highd}}
   \STATE Divide the $[0,1]$  interval along each dimension into intervals of length $\frac{1}{L}$. Then, choose a uniformly random offset $o$ from $\{0,1,2,\cdots,\frac{d}{\epsilon}\}\frac{1}{L}$. Then along each dimension, divide the length into alternating intervals of length $\frac{2}{L}$ and $\frac{d}{L\epsilon}$ with the interval at offset $o$ belong to the length $\frac{1}{L}$ interval. Let all the points belonging to intervals of length $\frac{1}{L}$ in any of the dimension be labelled as type 2 intervals and all other points as lying in type 1 intervals. One example of this partition is shown in Figure \ref{fig:partition-highd}.  Then Let $P$ be the partition induced i.e. the boundaries of the intervals. \\
   \STATE Sample a set $S = \{x_1,x_2,\cdots, x_M\}$ containing a total of $M = O(\frac{L^2}{\epsilon^4})$ unlabelled examples with distribution $\mathcal{D}$.\\
   \STATE \textbf{Output} $S, P$
   %\vspace{1.783cm}
   \label{algo:partition-highd}
   \end{algorithmic}
  \end{algorithm}
%
%
\begin{figure}
\centering
\begin{minipage}{.2\textwidth}
\centering
\includegraphics[width=1\linewidth]{partition1d.png}
\caption{.}
\label{fig:partition-1d}
\end{minipage}\qquad
\begin{minipage}{.2\textwidth}
\centering
\includegraphics[width=1\linewidth]{partition.png}
\caption{.}
\label{fig:partition-highd}
\end{minipage}
\end{figure}

\begin{theorem}
\label{thm:lipschitzlocalquery-highd}
Let $(x,y) \sim \mathcal{D}$ and let $F$ be the class of Lipschitz functions with Lipschitz constant atmost $L$. Then, there exists a $L$ Lipschitz function $\tilde{f}(x):[0,1]^d \rightarrow [0,1]$ such that $|E_{x,y \sim \mathcal{D}}|y-\tilde{f}(x)| - \min_{f \in F}E_{x,y \sim \mathcal{D}}|y-f(x)|| \leq \epsilon$ and for a fixed given $x \in [0,1]^d$, $\tilde{f}(x)$ can be computed with $O((\frac{L}{\epsilon})^d\frac{1}{\epsilon^3})$ unlabelled samples $x,y \sim \mathcal{D}$ and $O(\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d)$ label queries on those unlabelled samples.
\end{theorem}
%
\begin{proof}
Let $f^*(x)$ be the $L$ Lipschitz function with minimum error i.e. $$f^* = \arg\min_{f \in F} E_{x,y\sim \mathcal{D}}|y-f(x)|$$
%
%And let $\hat{f}$ be the function with the minimum error on data in $S$.
%$$\hat{f} = \arg\min_{f \text{ is } L \text{ Lipschitz} } \sum_i|y_i-f(x_i)|$$

Let $S, P = \text{Preprocess(L)}$ i.e. let $S$ be the set of the unlabelled samples given by Preprocess Algorithm and let $P$ be the partition given by the Preprocess algorithm. Let $S = \{x_1,x_2,\cdots,x_M\}$. Let the intervals of length $\frac{d}{L\epsilon}$ be labelled as type 1 intervals and intervals of length $\frac{1}{L}$ type 2 intervals. Let $\mathcal{D}_i$ be the conditional distribution of $\mathcal{D}$ on interval $I_i$.\\
%
Let $f^*_i:I_i \rightarrow [0,1]$ be the best $L$ Lipschitz function on an interval $I_i$ i.e. 
$$f^*_i = \arg\min_{f \text{ is } L \text{ Lipschitz} } E_{x,y\sim \mathcal{D}_i}|y-f(x)|$$
%
Let $f_i(x):I_i \rightarrow [0,1]$ be the best $L$ Lipschitz function learned using the labels of the unlabelled samples in $S$ lying in $I_i$ i.e.
%
$$f_i = \arg\min_{f \text{ is } L \text{ Lipschitz} } \sum_{j \in [M] \text{ such that } x_j \in I_i}|y_j-f(x_j)|$$
%
  Let $\mathcal{D}_{\text{type }1}$ and $\mathcal{D}_{\text{type }2}$ be the conditional distribution of $\mathcal{D}$ on intervals of type 1 and type 2 respectively.

Then by Lemma \ref{lemma:number_unlabelled_samples-highd}, we have with high probability, we have more than $\Omega(\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d)$ samples lying in all intervals of type 1 which have probability mass greater than $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ in them. Let us call the set of type 1 intervals having greater than $\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d$ unlabelled samples in them $G_1$. 
Hence, using Lemma~\ref{lemma:lipschitz_sample_complexity} where $l=\frac{d}{L\epsilon}$ we get that 
$$E_{x,y\sim \mathcal{D}_i}|f_i(x) - y| - E_{x,y\sim \mathcal{D}_i}|f^*_i(x) - y|\leq \epsilon \quad \forall \mathcal{D}_i \in G_1$$

%$$\frac{1}{M}\sum_{j \text{ such that } x_j \in I_i}|f_i(x) - y| \leq \frac{1}{M}\sum_{j \text{ such that } x_j \in I_i}|\hat{f}(x) - y|$$
%
Since, $f^*_i(x)$ is the best $L$ Lipschitz function on $I_i$, we get that 
$$E_{x,y\sim \mathcal{D}_i}|f^*_i(x) - y| \leq E_{x,y\sim \mathcal{D}_i}|f^*(x) - y| \quad \forall \mathcal{D}_i \in G_1$$
%

and hence, we get that  
\begin{align}E_{x,y\sim \mathcal{D}_i}|f_i(x) - y| - E_{x,y\sim \mathcal{D}_i}|f^*(x) - y|\leq \epsilon \quad \forall \mathcal{D}_i \in G_1 \label{eqn:error:type1-highd}
\end{align}

%
First of all, fix the values of the functions at the middle of the type 2 intervals to be $0$ for all type 2 slices along each dimension. For intervals say $I_i$ of type 2, let $f_i(x)$ be any $L$ Lipschitz function consistent with the functions $f_{i-1}(x)$ and $0$ at the boundaries of the interval. Note that it is always possible to obtain a function $f_i$ consistent at the boundaries since type $2$ intervals have length $\frac{2}{L}$ and therefore, an $L$ Lipschitz function can go from $0$ to $1$ in that interval by the Nonlinear Hahn-Banach theorem \url{https://web.math.princeton.edu/~naor/homepage%20files/embeddings_extensions.pdf}. 
%$$|f_i(x) - y| \leq 1$$
%
Now, let $\tilde{f}:[0,1]^d\rightarrow[0,1] = f_i(x) \text{ if } x \in I_i$ be disjoint union of the functions $f_i$ defined on disjoint intervals. Now, it is easy to see that $\tilde{f}(x)$ is a $L$ Lipschitz function since each of the individual $f_i(x)$ function is $L$ Lipschitz by construction and the functions $f_i(x)$ are consistent at the boundaries with each other.\\
%
Now, looking at the error rate of the function $\tilde{f}(x)$, combining this for all intervals of type $1$, we get that 
%
\begin{align*}
& E_{x,y\sim \mathcal{D} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D} }|f^*(x) - y|\\ &= Pr(x \in \text{  type }1 \text{ intervals} )(E_{x,y\sim \mathcal{D}_{\text{type }1} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D}_{\text{type }1} }|f^*(x) - y|)\\
&+ Pr(x\text{ lies in intervals of type } 2)(E_{x,y\sim \mathcal{D}_{\text{type }2} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D}_{\text{type }2} }|f^*(x) - y|)\\
%%%%
&= Pr(x \in \text{  type }1 \text{ intervals} )\sum_{i:I_i \text{ is a type 1 interval}}Pr(x \in I_i|x \in \text{type 1 intervals})(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|)) \\
&+ Pr(x\text{ lies in intervals of type } 2)(E_{x,y\sim \mathcal{D}_{\text{type }2} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D}_{\text{type }2} }|f^*(x) - y|)\\
%%%
&= \sum_{i:I_i \text{ is a type 1 interval}}Pr(x \in I_i)(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|)) \\
&+ Pr(x\text{ lies in intervals of type } 2)(E_{x,y\sim \mathcal{D}_{\text{type }2} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D}_{\text{type }2} }|f^*(x) - y|)\\
\end{align*}

Now, from Lemma~\ref{lemma:prob_intervals-highd}, we know that with probability at least $1-\epsilon$, a randomly sampled $x \sim \mathcal{D}$ lies in an interval of type 1. Moreover, for type 2 intervals, the worst case error can be $1$ since $\tilde{f},f$ are functions bounded between $[0,1]$. Hence, we get that

$Pr(x\text{ lies in intervals of type } 2)(E_{x,y\sim \mathcal{D}_{\text{type }2} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D}_{\text{type }2} }|f^*(x) - y|) \leq \epsilon\cdot1 = \epsilon$

Now computing the error bounds for intervals of type 1, we get that

\begin{align}
&\sum_{i:I_i \text{ is a type 1 interval}}Pr(x \in I_i)(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|))\nonumber\\ &= \sum_{i:I_i \text{ is a type 1 interval having number of samples }\geq \frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d \text{ and  probability mass }\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}}Pr(x \in I_i)(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|))\nonumber\\ 
&+ \sum_{i:I_i \text{ is a type 1 interval having number of samples }< \frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d \text{ and  probability mass }\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}}Pr(x \in I_i)(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|))\nonumber\\
&+ \sum_{i:I_i \text{ is a type 1 interval having probability mass }< \frac{\epsilon}{(\frac{L\epsilon}{d})^d}}Pr(x \in I_i)(E_{x,y\sim\mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|)) \label{eqn:combined-highd}
\end{align}

The total probability mass combined in type 1 intervals each having probability mass $\leq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ is upper bounded by $\epsilon$ because there are atmost $(\frac{L\epsilon}{d})^d$ intervals.
Also, in the worst case, the loss can be 1. Hence, we can get an upper bound of $\epsilon$ the third term of the equation \ref{eqn:combined-highd}.

Now, from Lemma~\ref{lemma:number_unlabelled_samples-highd}, we know that with high probability, the intervals which have probability mass $\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ and have $< \frac{1}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ unlabelled samples in them have total probability mass upper bounded by $\epsilon$. Also, in that case when we do not have enough samples in an interval, in the worst case, the loss would be 1. Hence, we get that

\begin{align*}
\sum_{i:I_i \text{ is a type 1 interval having number of samples }< \frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d\text{ and probability mass } \geq \frac{1}{L}}Pr(x \in I_i)(E_{x,y\sim \mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|))\leq\epsilon
\end{align*}

Now, we will calculate the error bound for all type 1 intervals. We know by equation~\ref{eqn:error:type1-highd} that $E_{x,y\sim \mathcal{D}_i}|f_i(x) - y| - E_{x,y\sim \mathcal{D}_i}|f^*(x) - y|\leq \epsilon \quad \forall \mathcal{D}_i \in G_1$ and the total probability mass is upper bounded by 1. Hence, we get that
\begin{align*}
\sum_{i:I_i \text{ is a type 1 interval having number of samples }\geq \frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d \text{ and probability mass } \geq \frac{1}{L}}Pr(x \in I_i)(E_{x,y\sim\mathcal{D}_i }(|\tilde{f}(x) - y| -  |f^*(x) - y|)) \leq \epsilon
\end{align*}
%
Combining the error bounds calculate above for all the intervals, we get that
%
\begin{align*}
E_{x,y\sim \mathcal{D} }|\tilde{f}(x) - y| - E_{x,y\sim \mathcal{D} }|f^*(x) - y| 
&\leq \epsilon+\epsilon +  \epsilon  = 3\epsilon
\end{align*}
%\begin{align*}
%|\frac{1}{M}\sum_{x_i,y_i \in S }|\hat{f}(x_i) - y_i| - E_{x,y\sim D }|\hat{f}(x) - y||
%&\leq \epsilon
%\end{align*}

%Also, since $M \geq \frac{L}{\epsilon^3}$, we know that 
%$E_{x,y\sim D }|\hat{f}(x) - y| - %E_{x,y\sim D }|f^*(x) - y| \leq %\epsilon$ by Lemma \ref{lemma:lipschitz_sample_complexity}.\\
%
%
This proves that $\tilde{f}(x)$ is atmost $3\epsilon$ worse than $f^*(x)$ in terms of the test error.\\
%
Also, note that for a given query point $x$, $\tilde{f}(x)$ can be computed by only querying the labels of the interval in which $x$ lies (in case if $x$ lies in a type 1 interval) or the two neighbouring intervals of the interval in which $x$ lies and hence, would only require $O(\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d)$ label queries.
%
\end{proof}
%
%
\begin{lemma}
\label{lemma:number_unlabelled_samples-highd}
When we sample $M = \Omega(\frac{1}{\epsilon^3}(\frac{L}{\epsilon})^d)$ unlabelled examples from the distribution $\mathcal{D}$, then with high probability $1-\delta$ the total mass of type 1 intervals each having probability mass $\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ having $\leq \Omega(\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d)$ unlabelled samples is upper bounded by $\epsilon$.
\end{lemma}
%
\begin{proof}
The expected number of samples that falls in an interval $I$ will probability mass greater than $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ is at least $\frac{1}{\epsilon^2}(\frac{d}{\epsilon^2})^d$. Using Chernoff bounds, we can get that $Pr(\text{number of samples in } I \leq \frac{1}{2\epsilon^2}(\frac{d}{\epsilon^2})^d) \leq e^{-\frac{d^d}{8\epsilon^{2(d+1)}}} \leq \epsilon$. Now, let $F_i$ be the event that $I_i$ interval which has probability mass $\geq \frac{\epsilon}{(\frac{L\epsilon}{d})^d}$ has $\leq \frac{1}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples in it. Now, we know that $F_i \leq \epsilon \forall i$ where $I_i$ is an interval of type 1 having probability mass greater than $\frac{\epsilon}{(\frac{L\epsilon}{d})^d}$. Now, the expected combined mass of type 1 intervals which have $\leq \frac{1}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples is $\sum_iPr(F_i)Pr(I_i) \leq \epsilon\sum_iPr(I_i) \leq \epsilon$. Now, using Markov's inequality, we get that with probability atleast $1-\delta$, the total mass of type 1 intervals having $\leq \frac{1}{2\epsilon^2}(\frac{d}{\epsilon^2})^d$ samples each is $\leq \frac{\epsilon}{\delta}$.  
\end{proof}
%
%
%
\begin{lemma}
\label{lemma:prob_intervals-highd}
When we divide the $[0,1]^d$ domain into type 1 and type 2 intervals as in the preprocessing step \ref{algo:partition-highd}, then with probability more than $1-\delta$, a randomly sampled $x\sim \mathcal{D}$ lies in intervals of type 1 or type 2 intervals have probability mass bounded by $\frac{\epsilon}{\delta}$ with probability $1-\delta$.
\end{lemma}
%
\begin{proof}
Now, we consider the division of every dimension i.e. $[0,1]$ independently into alternating intervals of length $\frac{d}{L\epsilon}$ and $\frac{1}{L}$ with the offset chosen uniformly randomly from $\{0, 1, 2, \cdots, \frac{d}{\epsilon}\}\frac{1}{L}$. For any set of fixed offsets chosen for the $d-1$ dimensions, the intervals of length $\frac{1}{L}$ chosen for the $dth$ dimension combined are disjoint in each of these divisions and together cover the entire $[0,1]^d$ and hence amount to probability mass $1$. Therefore, the total probability mass covered in the total $(\frac{d}{\epsilon})^d$ possible divisions is $d(\frac{d}{\epsilon})^{d-1}$.  Hence, there are atmost $\delta$ fraction out of the total $(\frac{d}{\epsilon})^d$ cases where the type 2 intervals have probability mass greater than $\frac{\epsilon}{\delta}$. Hence, with probability $1-\delta$, the type 2 intervals have probability mass upper bounded by $\frac{\epsilon}{\delta}$. %
\end{proof}
%

 \begin{algorithm}[H]
   \begin{algorithmic}[1]
\caption{Query($x, S, P=[\{b^i_0,b^i_1,b^i_2,\cdots\}]^d_{i=1}$)\label{alg5}}
    %\STATE S, P = Preprocess(L)
   \IF{query $x \in \text{type 1 interval say } I_J \text{ where } I_J(i) = [b^i_{J(i)-1}, b^i_{J(i)}]$}
   
   \STATE \textbf{Output} $f_J(x)$ where $f_J = \arg\min_{f \text{ is } L \text{ Lipschitz} } \sum_{x_j \in S \cap I_J}|y_j-f(x_j)|$\\

    \ELSIF{query $x \in \text{type 2 interval say } I_J$ where $I_J(i) = [b^i_{J(i)-1}, b^i_{J(i)}]$}
    %
       \FOR{$i=1$ to $d$}
   \IF{$[b^i_{J(i)-1}, b^i_{J(i)}]$ is a type 1 interval of dimension $i$}
   \STATE $C(i) = J(i)$ or $I_{C}(i) = [b^i_{J(i)-1}, b^i_{J(i)}]$
   \ELSE
   \IF{$|x_i-b^i_{J(i)-1}| \leq |x_i-b^i_{J(i)}|$}
   \STATE    $C(i) = J(i)-1$ or $I_{C}(i) = [b^i_{J(i)-2}, b^i_{J(i)-1}]$
   \ELSIF{$b^i_{J(i)} == 1$}
   \STATE $C = \phi$
   \STATE break out of for loop
   \ELSE
   \STATE    $C^i = J(i)+1$ or $I_{C}(i) = [b^i_{J(i)}, b^i_{J(i)+1}]$
   \ENDIF
   \ENDIF
   \ENDFOR
   \IF{$C \neq \phi$}
   \STATE \textbf{Output:} $f(x)$ where $f(x)$ is the Lipschitz extension of $f_C(x)$ with domain interval $I_C$ where $I_C(i) = [b^i_{C(i)-1}, b^i_{C(i)}] \quad i \in [d]$ to the superset $I_{C'}$ where $I_{C'}(i) = \left[\max{\left(0,\frac{b^i_{C(i)-2}+b^i_{C(i)-1}}{2}\right)}, \min{\left(\frac{b^i_{C(i)}+b^i_{C(i)+1}}{2},1\right)}\right] i \in [d]$ with constraints $f(x) = 1 \forall x \in I_{C'}$ if $x_i = \frac{b^i_{C(i)}+b^i_{C(i)+1}}{2},\frac{b^i_{C(i)-2}+b^i_{C(i)-1}}{2}$ for atleast one $i \in [d]$. 
    %
    \ELSE
    \STATE \textbf{Output:} 1
    \ENDIF
    %
\ENDIF
   %\vspace{1.783cm}
   \end{algorithmic}
  \end{algorithm}
